Design Of a Dual-band Patch Antenna with Stacked Structure

This project presents the design, simulation, and fabrication of a compact dual-band patch antenna using a stacked structure, targeting 2.25 to 2.35 GHz and 5.6 to 5.8 GHz ISM bands. A stacked configuration was chosen over a slotted design for its better performance, featuring two copper patches separated by dielectrics, with a single feed line and a 5 mm patch offset to enhance coupling. Simulations showed strong return loss and directional gain in both bands. Although physical testing was limited due to equipment constraints, the prototype met design expectations, demonstrating potential for use in compact wireless and embedded systems.

==> Preliminaries/3-dedication.tex <==
\begin{center}
\LARGE\textbf {Dedication}
\end{center}
\vspace{5pt}

If a dedication is included then it should be immediately after the Abstract page.\par
I don't what it is actually.
